A Socially Assistive Robot using Automated Planning in a Paediatric Clinical Setting

We present an ongoing project that aims to develop a social robot to help children cope with painful and distressing medical procedures in a clinical setting. Our approach uses automated planning as a core component for action selection in order to generate plans that include physical, sensory, and social actions for the robot to use when interacting with humans. A key capability of our system is that the robot's behaviour adapts based on the affective state of the child patient. The robot must operate in a challenging physical and social environment where appropriate and safe interaction with children, parents/caregivers, and healthcare professionals is crucial. In this paper, we present our system, examine some of the key challenges of the scenario, and describe how they are addressed by our system.

==> first_thoughts.tex <==
== Title:
* A Social Signal Aware Companion Robot using Automated Planning

== System Overview
* Properties of the scenario
* Components: planner, web-based GUI, sensors, interaction manager, Nao
* ROS integration

== Procedure Modelling
* Plan underpins interaction
* Robot behaviours: dance etc.
* Interaction: question answering
* Social Signal: Sensing patient state - anxious/engaged
* Procedure progression: Moving between different stages - are the necessary people in the room? Robot cueing the HCP - "The HCP is about to.."

== Transition Modelling: From Assumptions Based to Query Based
* Monitoring changes to world start is challenging.
* The system allows parameterisation so that each proposition can be associated with an alternative transition provider.
* In order to support early system testing -This has allowed us start data collection and receive feedback from practitioners.

== World Knowledge: From User Input to Sensing
* Predicting the world state in this setting is challenging (space, masks, internet, ...).
* Each type of information is associated with an input device.
* In practice, we have started with a web-based GUI for providing real-time information and are progressing to predictive models as the models are learned.

== Robustness:
* Challenging to close loop in this setting
* Challenging to predict the possible transitions
* Difficult to extract the actual state to allow recovery - e.g., implicit/abstract propositions


